Scalar Bosons and Supersymmetry

The recent discovery of a spin-0 Brout-Englert-Higgs boson leads to further enquire about other fundamental scalars. Supersymmetric theories involve, in relation with the electroweak breaking, five such scalars at least, two charged and three neutral ones, usually denoted as H$^\pm$, H, h and A. They also introduce spin-0 squarks and sleptons as the superpartners of quarks and leptons. Supersymmetric extensions of the standard model lead to the possibility of gauge/BEH unification by providing spin-0 bosons as extra states for spin-1 gauge bosons within massive gauge multiplets. Depending on its properties the 125 GeV boson observed at CERN may then also be interpreted, up to a mixing angle induced by supersymmetry breaking, as the spin-0 partner of the Z under two supersymmetry transformations, i.e. as a Z that would be deprived of its spin.

==> bourbaphydefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin of definition file AHPEFS.TEX                      %
% (c) Stephan Ammann, for Birkhaeuser, Dec 1999            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AHPDEFS.tex -- is red in by each header file             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\font\fxtit=cmssbx10 % For the new logo

\newcount\fpage\newcount\npage\newcount\lpage
\fpage=\fipage\npage=\nrpage
\lpage=\fpage\advance\lpage by\npage\advance\lpage by-1

\def\xrule{\vrule width2.25pt}
\def\yrule{\hrule height.5pt}
\def\yrulefill{\leaders\yrule\hfill}
\def\strutx{\vrule height8.5pt width0pt depth0pt}
\def\struty{\vrule depth3.5pt width0pt}
\def\strutz{\vrule height10.2pt width0pt}

\def\boxl{\vbox{\halign{##\hfil\cr
{\sc Le Boson H},  S{\'e}minaire Poincar{\'e} \volnr\  (\centnr\yearnr)
\the\fpage\ -- \the\lpage\cr
%\struty \copyright\ Birkh{\"a}user Verlag, Basel,
%\centnr\yearnr\cr
%1424-0637/\yearnr/\issuenr0\fipage-\the\npage\ \ %
%\$\,1.50$+$0.20/0\cr
}}}

\def\boxr{\vbox{\offinterlineskip
\halign{##\hfil\hskip1mm&##\hfil\cr
\noalign{\vskip.8mm}
\multispan2{\yrulefill}\cr
\xrule\strutz\struty
&\fxtit S{\'e}minaire Poincar{\'e}\cr
%\xrule\strutx&%
%\vbox to0pt{%
%\vbox to0pt{\vss\hbox{\fxtit and Applications NoDEA}}\vss}\cr
}}}

\def\titlebox{\vbox to0pt{\hsize=150mm\footnotesize\vss
\hbox to\hsize{\boxl\hfil\boxr}}}


\def\ps@myheadings{
\let\@mkboth\markboth
\def\@oddhead{\footnotesize {\sc Le Boson H},  \rm Vol. \volnr,  \centnr\yearnr
\hspace{6mm}\titletxt\hfil\thepage}%
\def\@oddfoot{} % % centered page number
\def\@evenhead{\footnotesize \thepage \hfil
\authortxt\hspace{6mm}S{\'e}minaire Poincar{\'e}}%
\def\@evenfoot{}%       % centered page number
}

\def\ps@plain{
\let\@mkboth\markboth
\def\@oddhead{%
\titlebox}%
\def\@oddfoot{}%      % centered page number
\def\@evenhead{}%
\def\@evenfoot{}%     % centered page number
}

\ps@myheadings              % 'myheading' page style
\pagenumbering{arabic}      % Arabic page numbers
\onecolumn                  % Single-column.

\setcounter{page}{\fpage}

\textwidth=150mm
\textheight=230mm
\parindent=8mm
\evensidemargin=.2cm
\oddsidemargin=1.2cm
\topmargin=0pt
\frenchspacing

\newcommand{\pdpg}{\postdisplaypenalty=-2000}
%% Used to force a page-break after a displayed equation

\let\dst=\displaystyle
\let\scr=\scriptstyle

\def\bfdefault{b}

\def\Rec{Received\ }
\def\Rev{Revised\ }

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of AHPDEFS.TEX                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of definition file

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% TeX-master: t
%%% TeX-master: t
%%% End: 

